Soundwave: Less is More for Speech-Text Alignment in LLMs

Existing end-to-end speech large language models (LLMs) usually rely on large-scale annotated data for training, while data-efficient training has not been discussed in depth. We focus on two fundamental problems between speech and text: the representation space gap and sequence length inconsistency. We propose Soundwave, which utilizes an efficient training strategy and a novel architecture to address these issues. Results show that Soundwave outperforms the advanced Qwen2-Audio in speech translation and AIR-Bench speech tasks, using only one-fiftieth of the training data. Further analysis shows that Soundwave still retains its intelligence during conversation. The project is available at https://github.com/FreedomIntelligence/Soundwave.

==> data_scaling_table.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lccr}
    \toprule
    Task & Ours 10k & Ours 1k \\
    \midrule
    \multicolumn{3}{c}{\textbf{ASR}~\ensuremath{\downarrow}} \\
    Librispeech-clean & \textbf{2.19} & 3.34 \\
    Librispeech-other & \textbf{5.05} & 6.86 \\
    MLS & \textbf{7.34} & 9.44 \\
    TED-LIUM & \textbf{7.03} & 11.41 \\
    Voxpupli & \textbf{10.28} & 13.76 \\
    Commonvoice & \textbf{13.86} & 21.39 \\
    \midrule
    \multicolumn{3}{c}{\textbf{AIR-Bench}~\ensuremath{\uparrow}} \\
    Speech Grounding & \textbf{59.2} & 25.2 \\
    Language Identification & \textbf{89.6} & 32.6 \\
    Gender Recognition & \textbf{90.3} & 66.8 \\
    Emotion Recognition & \textbf{60.5} & 24.6 \\
    Age Prediction & \textbf{58.9} & 50 \\
    Entity Recognition & \textbf{81.7} & 33.1 \\
    Intent Classification & \textbf{93.2} & 35.8 \\
    Speaker num. Verification & \textbf{73.3} & 24.6 \\
    Synthesized Detection & \textbf{72.5} & 51 \\
    Audio Grounding & 23.1 & \textbf{43.9} \\
    Sound Classification & \textbf{91.7} & 27.6 \\
    Acoustic Scene Classification & \textbf{83.8} & 24 \\
    Sound Question Answering & \textbf{49.7} & 39 \\
    \bottomrule
    \end{tabular}
    \caption{Overview of scaling performance comparisons.}
    \label{tab:performance_comparison}
\end{table}
